Automated Data Quality Validation in an End-to-End GNN Framework

Ensuring data quality is crucial in modern data ecosystems, especially for training or testing datasets in machine learning. Existing validation approaches rely on computing data quality metrics and/or using expert-defined constraints. Although there are automated constraint generation methods, they are often incomplete and may be too strict or too soft, causing false positives or missed errors, thus requiring expert adjustment. These methods may also fail to detect subtle data inconsistencies hidden by complex interdependencies within the data. In this paper, we propose DQuag, an end-to-end data quality validation and repair framework based on an improved Graph Neural Network (GNN) and multi-task learning. The proposed method incorporates a dual-decoder design: one for data quality validation and the other for data repair. Our approach captures complex feature relationships within tabular datasets using a multi-layer GNN architecture to automatically detect explicit and hidden data errors. Unlike previous methods, our model does not require manual input for constraint generation and learns the underlying feature dependencies, enabling it to identify complex hidden errors that traditional systems often miss. Moreover, it can recommend repair values, improving overall data quality. Experimental results validate the effectiveness of our approach in identifying and resolving data quality issues. The paper appeared in EDBT 2025.

==> Sections/old_section/introduction.tex <==
\section{Introduction}
The emergence of Big Data has marked a transformative phase in the digital age, presenting both novel opportunities and intricate challenges. Among these challenges, ensuring data quality is paramount, especially as data proliferates at an unprecedented rate in terms of volume, variety, and velocity. High-quality data is essential for reliable data-driven decision-making, particularly in machine learning applications where the integrity of training and test datasets directly impacts model performance. This paper explores the critical issue of data quality verification, focusing on innovative approaches that address the limitations of traditional methods.

\noindent\textbf{Background:} 
 In the context of Big Data, quality-aware systems have become indispensable tools. These systems aim to ensure that data adheres to specific quality benchmarks, regardless of its scale or diversity. Traditional quality-aware systems typically begin with data profiling, a process that generates metadata to describe various quality attributes such as missing values, data dependency rules, and other essential facets. This metadata forms the foundation for assessing data quality against established metrics and dimensions. However, traditional methods exhibit several significant limitations. They often rely heavily on expert-defined constraints, which are resource-intensive and time-consuming to develop and maintain. These constraints require substantial domain knowledge and manual effort for continuous monitoring and adjustment, making the process inefficient and prone to human error.

Moreover, some approaches attempt to automate constraint generation by learning from the dataset’s characteristics and data types. Despite these advancements, automatically set constraints are typically incomplete and may be either too stringent or too lenient. Strict constraints can lead to numerous false positives, flagging acceptable data as problematic, while lenient constraints may miss critical quality issues, allowing poor-quality data to pass through. Consequently, even automated systems require significant expert intervention to fine-tune and validate the constraints, limiting their practical effectiveness.

Additionally, traditional methods often fail to detect hidden relationships and dependencies within the data. Data quality is not only about individual data points but also about understanding the complex interrelationships among them. Traditional systems lack the capability to automatically recognize these latent connections, which can lead to the oversight of subtle yet crucial data quality issues. Experts, too, may overlook these hidden relationships, further compromising the data quality verification process.
% Quality-aware systems have risen to prominence as indispensable tools in the Big Data context. Their primary objective is to ensure that data, regardless of its scale or diversity, adheres to specific quality benchmarks. The vastness and complexity of Big Data amplify the need for such systems, as they serve as the first line of defense against potential quality discrepancies and anomalies that might otherwise go unnoticed in such a massive data landscape.

% A cornerstone of Quality-aware systems is their capability to model and measure data quality meticulously. This process is initiated with data profiling, a sophisticated technique that generates metadata. This metadata is not just a simple descriptor; it's a treasure trove of essential quality attributes, capturing nuances like missing values, data dependency rules, and other quality-related facets. Once armed with this rich metadata, the system is poised to conduct a thorough assessment, evaluating the data against a suite of established quality metrics and dimensions.

% Despite the advances in data quality verification, traditional quality-aware systems exhibit several significant limitations. Firstly, these methods often involve calculating various data quality dimensions and metrics or rely heavily on expert-defined constraints. This reliance on experts can be resource-intensive and time-consuming, as it demands substantial domain knowledge and manual effort to set appropriate constraints. Experts must continuously monitor and adjust these constraints to maintain data quality, which is not always feasible.

% Moreover, some approaches attempt to automate the constraint-setting process by learning from the dataset’s characteristics and data types. However, these automatically set constraints are typically not comprehensive enough. They either fail to cover all necessary aspects of data quality or set constraints that are too strict or too lenient. Strict constraints can lead to an excessive number of false positives, flagging acceptable data as problematic, while lenient constraints may miss critical quality issues, allowing poor-quality data to pass through. Consequently, these automated systems still require significant expert intervention to fine-tune and validate the constraints, limiting their practical effectiveness.

% Additionally, these traditional methods often fail to detect hidden relationships and dependencies within the data. Data quality is not only about individual data points but also about understanding the complex interrelationships among them. Traditional systems lack the capability to automatically recognize these latent connections, leading to potential oversight of subtle yet crucial data quality issues. Experts might also overlook these hidden relationships, further compromising the data quality verification process.

\noindent\textbf{Motivation:} The need for robust data quality verification has never been more critical in the era of Big Data. Traditional methods, while foundational, exhibit significant limitations that impede their effectiveness. These methods often depend heavily on expert-defined constraints, which can be incomplete, overly strict, or too lenient, requiring substantial domain knowledge and manual effort for continuous monitoring and adjustment. This dependence on experts not only makes the process resource-intensive and time-consuming but also introduces the risk of human error and oversight.

Moreover, automated approaches that attempt to learn constraints from the data itself often fall short. These automatically generated constraints frequently lack comprehensiveness, failing to cover all necessary aspects of data quality. They might also be miscalibrated, either too stringent, leading to numerous false positives, or too permissive, allowing poor-quality data to slip through. Consequently, these automated systems still necessitate significant expert intervention to fine-tune and validate the constraints, limiting their practical effectiveness.

A particularly challenging issue is the detection of hidden relationships and dependencies within the data. Traditional systems and even many automated approaches are not equipped to recognize these latent connections, which are crucial for identifying subtle yet significant data quality issues. Experts, too, may overlook these hidden relationships, further compromising the verification process.

These limitations underscore the urgent need for more advanced, automated methods that can provide comprehensive and accurate data quality verification without heavy reliance on expert input. Such methods must be capable of automatically detecting and leveraging hidden data relationships and dependencies, adapting to the diverse and growing scale of Big Data environments. This motivates the development of a novel approach that can address these critical challenges and enhance the overall efficacy and efficiency of data quality verification.

\noindent\textbf{Challenge:} Developing an advanced data quality verification system that addresses the limitations of traditional methods involves several significant challenges:
\textbf{Constraint-Free Identification:} Traditional methods rely on predefined constraints, which can be inaccurate. Our approach needs to automatically identify problematic data without such constraints, providing a more flexible and accurate solution.
\textbf{Hidden Relationship Detection:} Identifying latent relationships and dependencies within data is critical. Our method must effectively uncover and leverage these hidden patterns to ensure comprehensive data quality assessment.
\textbf{Reducing Expert Intervention:} Traditional systems require ongoing expert input for constraint management. Our solution aims to minimize this dependency, making the process more efficient and scalable.
\textbf{Scalability and Robustness:} The solution must handle large and complex datasets efficiently, maintaining performance and accuracy as data volume grows.

These challenges require a novel approach that combines advanced techniques for automatic data quality assessment, hidden pattern recognition, and scalability in Big Data environments.



\noindent\textbf{Our Solution:} In response to these challenges, we propose a novel approach for tabular data quality verification:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Knowledge Graph Generation:} Our method starts by automatically generating a knowledge graph from the original dataset. This graph captures intricate relationships and dependencies within the data that traditional methods might overlook.
    \item \textbf{Embedding Knowledge Graph:} The generated knowledge graph is then embedded with the tabular data. This embedding forms a comprehensive representation that integrates both the original data and its relational information.
    \item \textbf{Training the VAE:} We train a Variational Autoencoder (VAE) using the embedded data. The VAE learns to differentiate between problematic and non-problematic datasets by modeling the normal data distribution.
    \item \textbf{Error Identification:} By integrating the knowledge graph into the VAE framework, our approach can effectively identify specific samples that are likely to contain errors. This process enhances the detection of hidden data relationships and reduces the need for expert intervention.
\end{enumerate}
This novel approach addresses the key challenges by combining advanced techniques for automatic data quality assessment, hidden pattern recognition, and scalability in Big Data environments.


\noindent\textbf{Contributions:} The contributions of this paper are as follows:
\begin{enumerate}[leftmargin=*]
    \item We propose a novel approach that integrates automatically generated knowledge graphs with tabular data for enhanced data quality verification.
    \item We develop a VAE-based model that utilizes this combined representation to accurately identify and locate problematic data samples.
    \item We demonstrate that our method significantly reduces the reliance on expert-defined constraints and enhances the detection of hidden relationships within the data.
    \item We validate our approach through extensive experiments, showcasing its effectiveness and scalability in real-world Big Data scenarios.
\end{enumerate}

In the following sections, we delve deeper into the details of our approach, beginning with a comprehensive review of related work, followed by the methodology, experimental results, and conclusion.



==> Sections/old_section/relatedwork.tex <==
\section{RELATED WORK}
\label{sec:relatedwork}

Data quality is a critical area of research that focuses on ensuring datasets meet specific quality benchmarks to support accurate and reliable data analysis. Data quality profiling and assessment are fundamental components of this field. Data profiling generates metadata about data sources, capturing attributes such as data types, missing values, and distinct values. This metadata is essential for various applications, including data cleansing, data integration, and query optimization \cite{DBLP:journals/sigmod/Naumann13, oliveira2006data, abedjan2017data}. Profiling helps identify data quality issues, such as missing values, syntax violations, and referential integrity problems \cite{chiang2008discovering, ilyas2015trends, razniewski2011completeness}. The subsequent data quality assessment uses these profiling outputs to measure data quality dimensions like accuracy, completeness, and consistency, categorized into intrinsic, accessibility, contextual, and representational qualities \cite{DBLP:journals/jmis/WangS96, sidi2012data}. This assessment ensures that datasets adhere to quality standards, facilitating their effective use in various applications \cite{jayawardene2013curse, jayawardene2015analysis, YEGANEH201424}.


Addressing quality issues in ML pipelines is a field with growing interest in recent years. Several research works studied the relationship between data quality and ML-model performance, including the impact of data quality dimensions on ML algorithms \cite{Budach2022TheEO}, their link to MLOps \cite{renggli2021data,Xin2021ProductionML}, cleaning for ML \cite{DBLP:journals/corr/abs-1904-09483, krishnan2016activeclean} and quality verification of ML pipelines \cite{schelter2018automating}. The quality of an ML model is often related to the quality of the underlying data, namely training and serving data. This has led to proposed approaches for data preparation, like assessing data across various quality dimensions \cite{gupta2021data} and task-dependant quality assessment \cite{Foroni2021EstimatingTE}. Several approaches focused on the completeness of data \cite{karlavs2020nearest, schelter2020learning}. Others focus on the data drift between training and serving data. 

Data quality verification is essential for ensuring that datasets meet predefined quality standards before they are used for analysis or model training. Various studies have addressed different aspects of this topic. Fadlallah et al. \cite{fadlallah2023context}, Caveness et al. \cite{caveness2020tensorflow}, and Sinthong et al. \cite{sinthong2021dqdf} emphasize context-awareness, continuous ML pipelines, and data-quality-aware dataframes, yet they often depend on predefined rules and constraints that require expert intervention. Gu et al. \cite{bertino2018adaptive} and Li et al. \cite{li2022blindly} focus on visual data quality, presenting techniques that are not easily generalizable to other datasets. Schelter and colleagues \cite{schelter2018automating, schelter2019differential} explore automating data quality verification in large-scale scenarios but struggle with detecting hidden data relationships. Shrivastava et al. \cite{shrivastava2019dqa} introduce an interactive advisor for scalable data quality, yet it still relies heavily on expert-defined rules. These methods, while insightful, often fall short of providing fully automated, comprehensive solutions adaptable to various data types and scales without extensive expert input.





==> Sections/old_section/relatedwork__1_.tex <==
\section{RELATED WORK}
\label{sec:relatedwork}
Previous work in data quality research focuses on calculating data quality dimensions and statistics to evaluate data quality. Fundamental components of this research include data profiling and assessment.
% Data profiling generates metadata about data sources, capturing attributes such as data types, missing values, and distinct values. 
% This metadata is crucial for applications like data cleansing and integration~\cite{DBLP:journals/sigmod/Naumann13, oliveira2006data, abedjan2017data}. 
Profiling helps identify data quality issues, such as missing values and syntax violations~\cite{chiang2008discovering, ilyas2015trends, razniewski2011completeness}. Data quality assessment then uses these profiling outputs to measure dimensions like accuracy, completeness, and consistency~\cite{DBLP:journals/jmis/WangS96, sidi2012data}, ensuring datasets adhere to quality standards for various applications~\cite{jayawardene2013curse, jayawardene2015analysis, YEGANEH201424}.

% Data quality research ensures datasets meet specific benchmarks for accurate and reliable analysis. 
% Fundamental components include data profiling and assessment. 
% Data profiling generates metadata about data sources, capturing attributes like data types, missing values, and distinct values, crucial for applications such as data cleansing and integration~\cite{DBLP:journals/sigmod/Naumann13, oliveira2006data, abedjan2017data}. Profiling helps identify data quality issues, such as missing values and syntax violations~\cite{chiang2008discovering, ilyas2015trends, razniewski2011completeness}. 
% Data quality assessment uses profiling outputs to measure dimensions like accuracy, completeness, and consistency~\cite{DBLP:journals/jmis/WangS96, sidi2012data}, ensuring datasets adhere to quality standards for various applications~\cite{jayawardene2013curse, jayawardene2015analysis, YEGANEH201424}.

% Data quality is a critical area of research that focuses on ensuring datasets meet specific quality benchmarks to support accurate and reliable data analysis. Data quality profiling and assessment are fundamental components of this field. Data profiling generates metadata about data sources, capturing attributes such as data types, missing values, and distinct values. This metadata is essential for various applications, including data cleansing, data integration, and query optimization \cite{DBLP:journals/sigmod/Naumann13, oliveira2006data, abedjan2017data}. Profiling helps identify data quality issues, such as missing values, syntax violations, and referential integrity problems \cite{chiang2008discovering, ilyas2015trends, razniewski2011completeness}. The subsequent data quality assessment uses these profiling outputs to measure data quality dimensions like accuracy, completeness, and consistency, categorized into intrinsic, accessibility, contextual, and representational qualities \cite{DBLP:journals/jmis/WangS96, sidi2012data}. This assessment ensures that datasets adhere to quality standards, facilitating their effective use in various applications \cite{jayawardene2013curse, jayawardene2015analysis, YEGANEH201424}.

In ML pipelines, addressing quality issues has gained interest. Research has studied the relationship between data quality and ML performance, the impact of data quality dimensions on ML algorithms \cite{Budach2022TheEO}, their link to MLOps \cite{renggli2021data,Xin2021ProductionML}, and cleaning for ML \cite{DBLP:journals/corr/abs-1904-09483, krishnan2016activeclean}. The quality of ML models is related to the quality of the underlying data, leading to approaches for data preparation \cite{gupta2021data, Foroni2021EstimatingTE}, focusing on data completeness \cite{karlavs2020nearest, schelter2020learning} and data drift \cite{tahmasbi2020driftsurf,concept-drift-96}.
% Addressing quality issues in ML pipelines is a field with growing interest in recent years. Several research works studied the relationship between data quality and ML-model performance, including the impact of data quality dimensions on ML algorithms \cite{Budach2022TheEO}, their link to MLOps \cite{renggli2021data,Xin2021ProductionML}, cleaning for ML \cite{DBLP:journals/corr/abs-1904-09483, krishnan2016activeclean}. The quality of an ML model is often related to the quality of the underlying data, namely training and serving data. This has led to proposed approaches for data preparation, like assessing data across various quality dimensions \cite{gupta2021data} and task-dependant quality assessment \cite{Foroni2021EstimatingTE}. 
% Several approaches focused on the completeness of data \cite{karlavs2020nearest, schelter2020learning}. 
% Others focus on the data drift between training and serving data~\cite{tahmasbi2020driftsurf,concept-drift-96}.

Data quality verification is essential for ensuring datasets meet predefined quality standards before use in analysis or model training. 
Our method employs a feature graph~\cite{li2024graph} and Variational Autoencoder (VAE)~\cite{doersch2016tutorial} to detect hidden errors and automatically report specific problematic samples. 
While some studies use GNN and other ML models for data imputation~\cite{telyatnikov2023egg,cappuzzo2024relational,spinelli2020missing}, anomaly detection~\cite{du2022graph}, and Fraud Detection~\cite{rao2020xfraud,liu2021pick}, these methods are not being used for data quality validation. 
Most data quality validation work uses statistical methods or trains ML models with statistical information to detect data quality issues.
Fadlallah and Sinthong~\cite{fadlallah2023context,sinthong2021dqdf} emphasize context awareness and data-quality-aware dataframes but rely on predefined rules requiring expert intervention. Schelter et al.~\cite{schelter2018automating, schelter2019differential, caveness2020tensorflow} automate data quality verification in large-scale scenarios but struggle with hidden data relationships, they also used some statistic or simple ML methods to automatically generate constraints, but require expert fine-tuning. Shrivastava~\cite{shrivastava2019dqa} introduces an interactive advisor for scalable data quality but still relies heavily on expert-defined constraints. Redyuk~\cite{redyuk2021automating} trained the k-nearest neighbors (KNN)~\cite{peterson2009k} model to judge data quality using limited metrics, failing to detect many hidden errors and pinpoint specific problematic samples. %Bertino and Li~\cite{bertino2018adaptive,li2022blindly} focus on visual data quality with techniques not easily generalizable to other image datasets.

% Data quality verification is essential for ensuring that datasets meet predefined quality standards before they are used for analysis or model training. 
% Our method employs a feature graph~\cite{} and Variational Autoencoder (VAE)~\cite{} to detect hidden errors deeply and automatically report specific samples with issues. 
% While some studies use GNN and other ML models for data imputation~\cite{} and anomaly detection~\cite{}, these methods are not applied to data quality validation.

% Most data quality validation work uses statistical methods to verify data quality or use statistical information to train ML models for detecting data quality problems.
% \cite{fadlallah2023context,sinthong2021dqdf} 
% emphasize context awareness and data-quality-aware dataframes, yet they often depend on predefined rules and constraints that require expert intervention. 
% \cite{schelter2018automating, schelter2019differential, caveness2020tensorflow} explore automating data quality verification in large-scale scenarios but struggle with detecting hidden data relationships, they also used some statistic or simple ML methods to automatically generate constrains, but they constrains is not accuracy, need expert continue to fine-turn. 
% \cite{shrivastava2019dqa} introduces an interactive advisor for scalable data quality, yet it still relies heavily on expert-defined constraints. 
% \cite{redyuk2021automating} trained a k-nearest neighbors (KNN)~\cite{} model to judge data quality by computing limited quality metrics, which fails to detect many hidden errors, and their method cannot pinpoint which specific sample is incorrect.
% \cite{bertino2018adaptive,li2022blindly} focus on visual data quality, presenting techniques that are not easily generalizable to other image datasets. 
% for examples,

% Various studies have addressed different aspects of this topic. 

%Our method employs a feature graph and VAE to deeply detect some hidden errors, and it is fully automatic, capable of reporting which specific samples have issues.add some work using GNN and other Ml models to do the data imputation and anomaly detection, but there is no use for data quality validation, most of the work use statistic method of calculate statistic information the use statistic information to train a ml model to detect data quality problem, but these method just use not too much metrics to evaluate the quality, may lost some hidden error, and they can not report which sample have problem, because they calculate the metric for each feature, so they can not find which sample have problem, and these work also used ML model to detect the contains in the dataset. but not accuracy. need expert to fine-turn.

% Data quality verification is essential for ensuring that datasets meet predefined quality standards before they are used for analysis or model training. Various studies have addressed different aspects of this topic. 
% \cite{fadlallah2023context,caveness2020tensorflow,sinthong2021dqdf} 
% emphasize context awareness, continuous ML pipelines, and data-quality-aware dataframes, yet they often depend on predefined rules and constraints that require expert intervention. Gu et al. \cite{bertino2018adaptive} and Li et al. \cite{li2022blindly} focus on visual data quality, presenting techniques that are not easily generalizable to other datasets. Schelter and colleagues \cite{schelter2018automating, schelter2019differential} explore automating data quality verification in large-scale scenarios but struggle with detecting hidden data relationships. Shrivastava et al. \cite{shrivastava2019dqa} introduce an interactive advisor for scalable data quality, yet it still relies heavily on expert-defined rules. These methods, while insightful, often fall short of providing fully automated, comprehensive solutions adaptable to various data types and scales without extensive expert input.



%Fadlallah et al. \cite{fadlallah2023context}, Caveness et al. \cite{caveness2020tensorflow}, and Sinthong et al. \cite{sinthong2021dqdf} 

==> Sections/old_section/system_1.tex <==

\section{(Our Solution)}

In this section, we present our innovative approach for automated data quality validation and repair using advanced graph neural network techniques, with a particular focus on multi-task learning. Our solution is designed to efficiently detect both ordinary and hidden data quality issues, while also providing corrective suggestions for repairing identified errors. The key steps involved in our method are detailed below.

\subsection{Data Representation and Feature Graph Construction}

The first step in our approach is to represent the input tabular dataset as a graph. This representation helps in capturing intrinsic relationships between features, which is critical for identifying hidden errors that may not be detectable using traditional methods.

We begin by constructing a feature graph \$G = (V, E)\$, where each node \$v\_i \in V\$ represents a feature in the tabular dataset, and edges \$e\_{ij} \in E\$ represent dependencies or correlations between features \$v\_i\$ and \$v\_j\$. To construct the graph, we leverage a large language model (LLM) such as ChatGPT-4 to automatically infer meaningful relationships between features.

\noindent The process of using ChatGPT-4 for feature graph construction is as follows:

- **Input to ChatGPT-4**: We provide the LLM with feature names \$F = {f\_1, f\_2, \dots, f\_n}\$, their descriptions, and a random sample of 100 data points from the dataset. This input is structured as:

  \begin{itemize}
  \item **Feature Names (\$F\$)**: A list of feature names in the dataset.
  \item **Feature Descriptions (\$D\$)**: Detailed descriptions of each feature, which provide semantic information about the feature's purpose.
  \item **Sample Data Points (\$S\$)**: A subset of data points from the dataset to provide context on how features are related.
  \end{itemize}

  The input prompt provided to ChatGPT-4 is:
  \begin{quote}
  "Given the feature names, descriptions, and sample data points, determine the relationships between features. Provide the relationships in JSON format, where each key-value pair represents a pair of features and the type of relationship between them."
  \end{quote}

- **Output from ChatGPT-4**: The model generates a JSON file capturing feature relationships, which is then parsed to construct the feature graph. The relationships are represented as:

  indicating that there is a relationship between features \$f\_i\$ and \$f\_j\$.

Using these relationships, we construct the knowledge-based feature graph \$G = (V, E)\$, where \$V\$ represents features and \$E\$ represents edges indicating relationships between features.

\subsection{Graph Neural Network Encoder}

Once the feature graph is constructed, we employ a Graph Neural Network (GNN) to learn a latent representation of the features. The goal is to capture the underlying structure of the clean dataset and learn meaningful feature embeddings that can be used for data validation and repair.

We use a hybrid Graph Attention Network (GAT) and Graph Isomorphism Network (GIN) encoder to effectively model both the feature-level attention and the feature aggregation:

\begin{itemize}
\item \textbf{Graph Attention Network (GAT)}: The GAT layer learns attention coefficients for each node's neighbors, allowing the model to focus on the most relevant features during aggregation. The output of the GAT layer for node \$v\_i\$ is given by:
\begin{equation}
h\_i^{(l+1)} = \sigma\left( \sum\_{j \in \mathcal{N}(i)} \alpha\_{ij}^{(l)} W^{(l)} h\_j^{(l)} \right),
\end{equation}
where \$\alpha\_{ij}^{(l)}\$ are the learned attention coefficients, \$W^{(l)}\$ is the weight matrix, \$\mathcal{N}(i)\$ represents the neighbors of node \$i\$, and \$\sigma\$ is a non-linear activation function. The GAT layer helps the model focus on the most important relationships by assigning different attention weights to different neighbors, which is crucial for capturing complex dependencies between features.

```
\item \textbf{Graph Isomorphism Network (GIN)}: The GIN layer aggregates feature information by summing the features from neighboring nodes, followed by a multi-layer perceptron (MLP). This allows for stronger feature aggregation. The output for node $v_i$ is given by:
\begin{equation}
h_i^{(l+1)} = \text{MLP}^{(l)}\left( (1 + \epsilon) h_i^{(l)} + \sum_{j \in \mathcal{N}(i)} h_j^{(l)} \right),
\end{equation}
where $\epsilon$ is a learnable parameter or fixed scalar. The GIN layer is effective in capturing structural information and distinguishing different graph structures, making it useful for learning robust feature embeddings.
```

\end{itemize}

\noindent \textbf{Combining GAT and GIN:} The GAT and GIN layers are combined sequentially to leverage the strengths of both models. First, the GAT layer is applied to focus on the most relevant neighboring features through attention mechanisms. Then, the GIN layer is used to aggregate information from these neighbors in a more expressive manner, capturing both the attention-based relevance and the structural properties of the graph. This combination allows us to learn a comprehensive representation of each feature that incorporates both its importance (through GAT) and its structural context (through GIN).

The final output of the GNN encoder is a latent representation matrix \$Z \in \mathbb{R}^{n \times d}\$, where \$d\$ is the embedding dimension. The model is trained using the clean dataset, and the loss function used is Mean Squared Error (MSE) between the reconstructed feature values and the original values, ensuring that the learned embeddings accurately represent the clean data structure.

\subsection{Multi-Task Decoder for Data Quality Validation and Repair}

Our solution incorporates a multi-task learning framework to simultaneously perform data quality validation and data repair.

The multi-task decoder consists of two main components:

\begin{itemize}
\item \textbf{Data Quality Validation Decoder}: The first task is to validate the data quality by reconstructing the feature embeddings. Given the latent representation \$Z\$, we apply a reconstruction layer to predict the original feature values:
\begin{equation}
\hat{X}*{\text{validation}} = W*{\text{validation}} Z + b\_{\text{validation}},
\end{equation}
where \$W\_{\text{validation}}\$ and \$b\_{\text{validation}}\$ are learnable parameters. The reconstruction error \$L\_{\text{validation}}\$ is used to detect potential data quality issues.

```
\item \textbf{Data Repair Decoder}: The second task is to repair detected errors by generating corrected feature values. We use an additional MLP-based decoder to map the latent representation $Z$ to repaired feature values:
\begin{equation}
\hat{X}_{\text{repair}} = W_{\text{repair}} Z + b_{\text{repair}},
\end{equation}
where $W_{\text{repair}}$ and $b_{\text{repair}}$ are learnable parameters. The repair loss $L_{\text{repair}}$ is used to train the model to generate realistic corrected values for erroneous entries.
```

\end{itemize}

We define a combined loss function to optimize both tasks simultaneously:
\begin{equation}
L = \lambda\_{\text{validation}} L\_{\text{validation}} + \lambda\_{\text{repair}} L\_{\text{repair}},
\end{equation}
where \$\lambda\_{\text{validation}}\$ and \$\lambda\_{\text{repair}}\$ are hyperparameters that balance the contributions of the validation and repair tasks.

The model is trained using the Adam optimizer with a learning rate of \$0.01\$, and training is performed for 50 epochs. The training process involves feeding batches of clean data through the GNN encoder and multi-task decoder, and updating the parameters based on the combined loss function.

\subsection{Threshold-Based Anomaly Detection}

After training, we use the validation set to determine a threshold for detecting data quality issues. The reconstruction error for each instance in the validation set is computed as follows:
\begin{equation}
E\_i = | X\_i - \hat{X}*{\text{validation}, i} |^2,
\end{equation}
where \$X\_i\$ represents the original feature values and \$\hat{X}*{\text{validation}, i}\$ represents the reconstructed values. We set the anomaly threshold \$T\$ to the 95th percentile of the reconstruction errors in the validation set:
\begin{equation}
T = \text{quantile}*{0.95}(E*{\text{validation}}).
\end{equation}
Instances with reconstruction errors exceeding this threshold are flagged as potentially problematic.

\subsection{Data Quality Evaluation and Repair}

Once the model is trained and the quality threshold is established, we proceed to evaluate the quality of data in test sets and perform data repair where necessary. The evaluation and repair process involves the following steps:

The trained model is applied to two test sets: a clean test set (Test Set 1) and a dirty test set (Test Set 2). For each test instance, we compute the reconstruction error using the validation decoder:
\begin{equation}
E\_i = | X\_i - \hat{X}*{\text{validation}, i} |^2,
\end{equation}
where \$X\_i\$ represents the original feature values, and \$\hat{X}*{\text{validation}, i}\$ represents the reconstructed values. If the reconstruction error exceeds the threshold \$T\$, the instance is flagged as potentially problematic.

For instances flagged as problematic, we use the repair decoder to generate corrected feature values. The repaired data \$\hat{X}*{\text{repair}}\$ is computed as:
\begin{equation}
\hat{X}*{\text{repair}} = W\_{\text{repair}} Z + b\_{\text{repair}},
\end{equation}
where \$W\_{\text{repair}}\$ and \$b\_{\text{repair}}\$ are learnable parameters from the repair decoder. These corrected values are used to replace the erroneous entries in the dataset.

For each erroneous feature \$f\_j\$ of instance \$X\_i\$, the repaired value is given by:
\begin{equation}
\hat{x}*{ij} = \hat{X}*{\text{repair}, i, j},
\end{equation}
where \$\hat{x}\_{ij}\$ represents the repaired value for feature \$f\_j\$ in instance \$i\$. These repair suggestions are logged for further inspection and manual verification by domain experts if needed.

We evaluate the effectiveness of our approach using metrics such as accuracy of error detection, precision, recall, and the quality of the repair suggestions. The clean test set (Test Set 1) is used to verify the model's false positive rate, while the dirty test set (Test Set 2) is used to evaluate the true positive rate and repair accuracy.

Through these steps, our approach provides a comprehensive solution for not only detecting data quality issues but also suggesting and applying corrections, thereby improving the overall reliability of the dataset.

==> Sections/old_section/systems.tex <==
\section{OUR APPROACH: DQuaG}

\begin{figure*}[tb]
\centering
\includegraphics[width=0.75\textwidth]{Figures/framework_adqv.png}
\vspace{-0.6\baselineskip}
\caption{Data Quality Validation Framework Using GNN and VAE. Top: Training on clean data for Approach Establishment. Bottom: Validating unseen datasets by reconstruction error comparison.}
\vspace*{-0.3cm}
%\soror{highlight in the caption the process at the top and the one at the bottom of teh figure }
\label{fig:framework}
\end{figure*}

%In this section, we detail our novel approach to automated data quality validation using graph representation learning and a Variational Autoencoder (VAE) framework. Assuming we start with a clean dataset, our method addresses the limitations of traditional data quality verification techniques through a series of steps designed to capture intrinsic relationships within tabular data and assess data quality with minimal expert intervention.


In this section, we present DQuaG (Data Quality Graph), a novel approach for data quality validation. 
Figure~\ref{fig:framework} illustrates the framework of our approach, which includes both the training process using a clean dataset to train the GNN and VAE, and the data quality validation process using these trained models. 
%\qw{For the training phase, }
%\qw{For the validation phase, }

Note that DQuaG requires a clean dataset to train its models, which is a common assumption when embracing VAE in relevant problems.
The clean dataset serves as the foundational benchmark for our model, providing a reference state of high data quality against which data errors are identified. 
%This dataset is not only used to train the GNN and VAE models, but also to define a normative baseline for what constitutes acceptable data quality.

% \subsection{Training GNN and VAE on Clean Data for Data Quality Validation}
\subsection{Training GNN and VAE on Clean Data}
\subsubsection{\textbf{Feature Graph Construction}}

The initial step in our approach involves constructing a feature graph from clean tabular data to capture intrinsic relationships and dependencies between data features.
First, we address the challenge of diverse data types: categorical variables are transformed using label encoding, and timestamp data is broken into components (i.e., day, month, year). 
This uniform input format is critical for graph-based processing.

We then use ChatGPT-4~\cite{openai2024gpt4} to automate the feature graph construction. 
Given a clean dataset, we extract the feature names \( F \) and their descriptions \( D \) from the data source. We then randomly sample 100 data points from the dataset, denoted as \( S \). These feature names, descriptions, and sample data points are provided to the ChatGPT-4, structured as follows: \(\text{Input} = \{ F, D, S \}\), then ChatGPT-4 generates a JSON file capturing feature relationships.
The output format is \(\text{Feature\_Relationships} = \{ (f_i, f_j) \mid f_i, f_j \in F \}\), indicating that there is a relationship between features \( f_i \) and \( f_j \).

Using these relationships, we construct the knowledge-based feature graph \( G = (V, E) \), where \( V \) represents features and \( E \) represents edges indicating relationships between features.

% \subsubsection{\textbf{Feature Graph Construction}}

% The initial step in our methodology involves constructing a feature graph from clean tabular data, which is essential for capturing the intrinsic relationships and dependencies between different data features.

% To facilitate this process, our approach first addresses the challenge of handling diverse data types. 
% In the preprocessing stage, categorical variables are transformed using label encoding, which assigns each unique category a unique integer based on alphabetical ordering. 
% For timestamp data, we extract significant components such as day, month, and year. 
% This uniform input format is critical for the subsequent graph-based processing. 

% Following the preprocessing, we utilize a large language model, ChatGPT-4 \cite{openai2024gpt4}, to automate the construction of the feature graph. This integration allows for a more nuanced capture of feature relationships and dependencies, reducing reliance on expert knowledge and manual effort.

% Given a clean dataset, we extract the feature names \( F = \{f_1, f_2, \ldots, \\f_n\} \) and their descriptions \( D = \{d_1, d_2, \ldots, d_n\} \) from the data source. We then randomly sample 100 data points from the dataset, denoted as \( S = \{s_1, s_2, \ldots, s_{100}\} \). These feature names, descriptions, and sample data points are provided to the LLM, structured as follows: \(\text{Input} = \{ F, D, S \}\).

% The LLM analyzes the provided input and generates a structured JSON file capturing the relationships between features. The output format is \(\text{Feature\_Relationships} = \{ (f_i, f_j) \mid f_i, f_j \in F \}\), indicating that there is a relationship between features \( f_i \) and \( f_j \).

% Using the relationships provided by the LLM, we construct the feature graph \( G = (V, E) \) where \( V = F \) (nodes representing features) and \( E = \{(f_i, f_j) \mid (f_i, f_j) \in \text{Feature\_Relationships} \} \) (edges representing relationships). 

%----------------------------
%This graph-based representation allows us to model complex interdependencies within the data that are often overlooked by traditional methods, enhancing our ability to perform thorough data quality assessments.



% \subsubsection{\textbf{Training the Graph Neural Network (GNN) and Representing the Clean Dataset}}
\subsubsection{\textbf{Training GNN and preparing training data for VAE}}

Once the feature graph is constructed, we train a Graph Convolutional Network (GCN)~\cite{zhang2019graph} to generate feature embeddings. 
The GCN processes both the feature graph \( G = (V, E) \) and the original tabular data. Assume each instance in the original tabular data is an \( n \)-dimensional tuple \( \mathbf{x} \in \mathbb{R}^n \).

The GCN leverages the feature graph to learn the intrinsic relationships between features and produces embeddings that reflect the underlying structure of the clean data. Specifically, for each instance \( \mathbf{x} \), the GCN generates an \( n \)-dimensional embedding \( \mathbf{z} \in \mathbb{R}^n \). 
%This embedding \( \mathbf{z} \) captures the information from each feature's value and incorporates the relationships between features as learned from the feature graph.
% We train the GCN using the Adam optimizer, which is well-suited for handling graph-based data. The loss function used during training is the mean-squared error (MSE) between the predicted and true values for a set of labeled data. 
Formally, let \( \mathbf{Z} \) be the matrix of embeddings, where each row \( \mathbf{z}_i \) corresponds to an instance \( \mathbf{x}_i \). 
The GCN updates the embeddings by aggregating information from neighboring nodes in the feature graph, ensuring that the final embedding \( \mathbf{z}_i \) incorporates both the feature values and the relationships between features.

%These embeddings \( \mathbf{Z} \) serve as a compact and informative representation of the data's quality attributes, providing a robust basis for subsequent data quality assessment.


% \subsubsection{\textbf{Training the VAE for Encoding and Decoding}}
\subsubsection{\textbf{Training the VAE}}
%\qw{the input of VAE is composed by both the original data and the GNN output, i.e., move the above embedding part here}
The feature embeddings \( \mathbf{Z} \) generated by the GNN are then used to train a Variational Autoencoder (VAE). 
The VAE consists of an encoder and a decoder. The encoder maps the embeddings \( \mathbf{z} \) into a latent space, and the decoder reconstructs the embeddings back to their original feature space. This training is performed using the embeddings from the clean data, allowing the VAE to learn a probabilistic model of the normal data distribution.

\subsubsection{\textbf{Collecting the statistics of reconstruction errors}}
During training, we record the reconstruction error for each instance. The reconstruction error is essentially the loss for each instance. This results in a list of reconstruction errors, \(\mathcal{E}\). Given that even cleaned datasets may contain undetected errors, we do not set the maximum reconstruction error as the threshold for identifying problematic instances. Instead, we set the threshold at the 95th percentile of \(\mathcal{E}\), denoted as \( e_{clean} \). Instances with reconstruction errors above \( e_{clean} \) are flagged as potentially problematic.

%\qw{adjsut this paragraph}
%This process ensures that the VAE effectively learns the characteristics of the clean data while providing a robust method for detecting deviations from the norm in new datasets.


\subsection{Data Quality Validation Process}

\noindent{\textbf{Detecting Data Quality Issues by Reconstruction Errors}.}
With the GNN and VAE trained on the embeddings of the clean data, we proceed to assess the quality of new, unseen datasets. These unseen datasets must keep the same schema as the original clean dataset. The process involves several steps.
First, we generate embeddings for the new dataset using the trained GNN. Let \( \mathbf{Z}_{\text{new}} \) be the embeddings of the new dataset instances. These embeddings are then input into the trained VAE to obtain a list of reconstruction errors, denoted as \(\mathcal{E}_{\text{new}}\).
Next, we compare each reconstruction error in \(\mathcal{E}_{\text{new}}\) with the threshold \( e_{clean} \) from the clean dataset. 
We calculate the proportion of instances in the new dataset with reconstruction errors exceeding \( e_{clean} \), denoted as \( R_{error} \). 
Since the threshold was set at the 95th percentile for the clean dataset, we expect around 5\% of clean data instances to exceed this value. 

To account for data variability, if \( R_{error} \) exceeds \( 5\% \times n \), we classify the new dataset as problematic. This means if more than \( 5n\% \) of instances in the new dataset have errors greater than \( e_{clean} \), we will report the dataset has data quality issues. The parameter \( n \) can be adjusted based on observed reconstruction errors after deployment.
In our experiments, we set \( n = 1.2 \), which exhibited good performance.
Finally, we report the indices of all instances in the new dataset with reconstruction errors above \( e_{clean} \), clearly identifying problematic samples.

% Next, we compare each reconstruction error in \(\mathcal{E}_{\text{new}}\) with the previously determined threshold \( e_{cleaned} \). We calculate the proportion of instances in the new dataset that have reconstruction errors exceeding \( e_{cleaned} \), denoted as \( R_{error} \). Since the threshold was set at the 95th percentile for the clean dataset, it is expected that approximately 5\% of the clean dataset instances would have reconstruction errors above this threshold.
% To account for data variability, if \( R_{error} \) exceeds \( 5\% \times n = 5n\% \), we classify the new dataset as problematic. This means that if more than 5n\% of the instances in the new dataset have reconstruction errors greater than \( e_{cleaned} \), the dataset is flagged as having data quality issues.

% Finally, we report the indices of all instances in the new dataset that have reconstruction errors above \( e_{cleaned} \), providing a clear indication of which specific samples are problematic.

%This process allows us to effectively detect data quality issues in new datasets, capturing both explicit errors and subtle inconsistencies that traditional approaches may miss.


\noindent{\textbf{Detecting Feature Errors}.}
Each instance's reconstruction error \( e \) is a list corresponding to each feature's loss. To identify specific problematic features, we detect outliers with significantly higher reconstruction errors.
For an instance \( \mathbf{x}_i \), let \( \mathbf{e}_i = [e_{i1}, e_{i2}, \ldots, e_{in}] \) be the reconstruction errors for the \( n \) features. We calculate the mean \( \mu_i \) and standard deviation \( \sigma_i \) of the errors. Features with errors greater than \( \mu_i + 5\sigma_i \) are flagged as problematic.

%By reporting these outlier features, we can pinpoint which specific parts of an instance contribute most to data quality issues. 
This drill-down process helps identify exact feature-level problems within instances, facilitating targeted data cleaning.


%Our approach offers several key advantages over traditional data quality verification methods. By leveraging GNNs and VAEs, it automatically identifies data quality issues without predefined constraints and detects hidden relationships within the data. This reduces the need for continuous expert input, making the process more efficient and scalable. Additionally, it can pinpoint problematic samples and specific features, facilitating targeted data cleaning and correction.





